Buying Privacy: User Perceptions of Privacy Threats from Mobile Apps

As technology and technology companies have grown in power, ubiquity, and societal influence, some companies -- and notably some mobile apps -- have come to be perceived as privacy threats. Prior work has considered how various factors impact perceptions of threat, including social factors, political speech, and user-interface design. In this work, we investigate how user-visible context clues impact perceptions about whether a mobile application application poses a privacy threat. We conduct a user study with 2109 users in which we find that users depend on context clues -- such as presence of advertising and occurrence (and timing of payment) -- to determine the extent to which a mobile app poses a privacy threat. We also quantify how accurately user assessments match published data collection practices, and we identify a commonly-held misconception about how payments are processed. This work provides new insight into how users assess the privacy threat posed by mobile apps and into social norms around data collection.

==> figures/old/trustToAssessment.tex <==
\begin{figure}[t!]
      \includegraphics[width = \columnwidth] {figures/assessmentByTrust.pdf}
      \caption{Distribution of Data Assesment by Trust Level (out of 19 possible types of data). Green triangles show the mean, yellow lines show the median, boxes show interquartile range, and whiskers show from 5\% to 95\%.}
      \label{fig:directManipulationBoxplot}
\end{figure}

==> sections/40-results-old.tex <==
\section{Results}

Analysing the data from our user studies led to two key results. We found that trust affects user assessment of unnecessary data collection by a mobile game app, and we identified and validated several signals---data collection, reputation, advertising, and payment---that influence user trust in this context.


% \subsection{Trust Affects Assessment of Unnecessary Data Collection }
% \label{sec:results-trust->collection}

% \begin{figure}

%     \begin{tabular}{lr}
%     \hline
%      Condition                             &   Mean Yeses \\
%     \hline
%      very trustworthy                      &      3.68932 \\
%      somewhat trustworthy                  &      4.35052 \\
%      neither trustworthy nor untrustworthy &      4.12245 \\
%      somewhat untrustworthy                &      6.78095 \\
%      very untrustworthy                    &      9.16    \\
%     \hline
%     \end{tabular}
%     \caption{Average Data Assessment by Trust Level (out of 19 possible types of data)\label{tab:directManipulationMeans}}
% \end{figure}
% Note: I'm not sure we need this table, as the information is depicted in the following figure



\subsection{The Effect of Trust on on Beliefs about Unnecessary Data Collection}

In our first user study, participants were told how trustworthy they considered a mobile game app and asked to infer which types of data the app would collect (following the methodology described in Section~\ref{subsec:trust->collection}). The reported data collection assessment by trust level, adjusted to include only unnecessary data collection, is summarized in Figure~\ref{fig:directManipulationBoxplot}. $p$\mbox{-}values from two-sample pairwise $t$-tests are given in Figure~\ref{table:pairwise-pvals}.



We found that participants assigned to low-trust conditions (somewhat untrustworthy and very untrustworthy) assumed that significantly more unnecessary data collection would occur compared to participants assigned to high-trust conditions (somewhat trustworthy and very trustworthy). Participants in low-trust conditions predicted an average of 7.94/19 types of data would be unnecessarily collected, whereas participants in high-trust conditions predicted an average of 4.01/19 types of data would be unnecessarily collected. We used a two-sample t-test to confirm that these means are significantly different ($p =1.940e{-15}$). \footnote{We chose to use t-tests as they are robust to the normality assumption, particularly with large sample sizes, which were present in this study. As possible data points are limited in range (maximum 19 pieces of data to be collected) there were also few outliers that could significantly affect t-tests, further making them a good choice.} 
% TODO: add numbers to this paragraph
% Question: did we run a regression on this?
% Consider adding a just somewhat un vs both trustworthy




Notably, participants assigned to the very untrustworthy condition assessed particularly high levels of data collection compared to the other conditions. The mean number of data types assessed by participants in this condition was $35\%$ higher than in the next-highest (somewhat untrustworthy) condition, and is confirmed to be significantly different using two-sample t-test ($p=0.00204$). Moreover, 75\% of participants in the very untrustworthy condition inferred that at least 6 different types of data were collected, whereas for all other conditions, the 75th percentile was no more than two types of data. We hypothesize that this might imply certain underlying beliefs, such as the belief that only ``sketchy'' or actively malicious apps are likely to collect large amounts of data. 
%\todo{Look at individual types of data?}.

\input{figures/trustToAssessment} 

\begin{comment}
\begin{figure*}
\begin{center}
\begin{tabular}{ |c||c|c|c|c|c| } 
 \hline
 \parbox{2.5cm}{\centering Trust Level} & \parbox{2.5cm}{\centering Very \\ Untrustworthy} & \parbox{2.5cm}{\centering Somewhat\\ Untrustworthy} & \parbox{2.5cm}{\centering Neither Trustworthy nor Untrustworthy} & \parbox{2.5cm}{\centering Somewhat \\Trustworthy} & \parbox{2.5cm}{\centering Very \\Trustworthy} \\ 
 \hline
 \hline
 \parbox{2.5cm}{\centering Very \\ Untrustworthy} & NA & 0.00204 & 2.80E-12 & 1.76E-11 & 4.43E-14\\ 
 \hline
 \parbox{2.5cm}{\centering Somewhat\\ Untrustworthy} & & NA & 6.90E-05 & 0.000249 & 3.94E-06\\
 \hline
 \parbox{2.5cm}{\centering Neither Trustworthy nor Untrustworthy} &  &  & NA & 0.670 & 0.427\\
 \hline
 \parbox{2.5cm}{\centering Somewhat \\Trustworthy} &  &  &  & NA & 0.222\\
 \hline
 \parbox{2.5cm}{\centering Very \\Trustworthy} &  &  &  &  & NA\\ 
 \hline
\end{tabular}
\caption{Results of Two-sample t-test p-values for Different Assigned Trusts}
\label{table:pairwise-pvals}
\end{center}
\end{figure*}
\end{comment}

\begin{figure}
\begin{center}
{\small
\begin{tabular}{ |c||c|c|c|c|c| } 
 \hline
 \parbox{1cm}{\centering Trust } & \parbox{1cm}{\centering Very \\ Untrust.} & \parbox{1cm}{\centering Some.\\ Untrust.} & \parbox{1cm}{\centering Neither} & \parbox{1cm}{\centering Some. \\Trust.} & \parbox{1cm}{\centering Very \\Trust.} \\ 
 \hline
 \hline
 \parbox{1cm}{\centering Very \\ Untrust.} & NA & 0.00204 & 2.80e-12 & 1.76E-11 & 4.43E-14\\ 
 \hline
 \parbox{1cm}{\centering Some.\\ Untrust.} & & NA & 6.90e-05 & 0.000249 & 3.94E-06\\
 \hline
 \parbox{1cm}{\centering Neither} &  &  & NA & 0.670 & 0.427\\
 \hline
 \parbox{1cm}{\centering Some. \\Trust.} &  &  &  & NA & 0.222\\
 \hline
 \parbox{1cm}{\centering Very \\Trust.} &  &  &  &  & NA\\ 
 \hline
\end{tabular}
}
\caption{Results of Two-sample t-test p-values for Different Assigned Trusts}
\label{table:pairwise-pvals}
\end{center}
\end{figure}

However, there were not statistically significant differences between the two high-trust conditions ($p=0.222$) or between the combined high-trust conditions (very trustworthy somewhat trustworthy) and the neutral condition ($p=0.811$). We hypothesize that the diminished effect of trust on assessment at higher trust levels might be due to the fact that our studies looked specifically at game apps: users might place an a priori upper bound on the level of trustworthiness they ascribe to game apps. Thus our participants, who were told that the app in question was a game, may be likely to be reasoning from a compressed scale of internal feelings about trustworthiness. This hypothesis is consistent with the results from the study looking at the effect of ads and payment, which found that just $8.33\%$ of participants who were shown screenshots from a real-world mobile game app (a free app containing ads) rated that app as very trustworthy (a complete description of the results of that study is available in Section~\ref{subsec:results:ads->trust}).


We also found that the neutral trust condition did not fit the trend defined by the four non-neutral conditions. % This is not a technically meaningful sentence. TODO: discuss whether there are statistics to support this story. 
We hypothesize that participants in this condition might be interpreting the phrase ``neither trustworthy nor trustworthy'' ambiguously, imposing assumptions about the general trustworthiness of apps more strongly than in other conditions.



\subsection{Signals that Influence Trust}



In our follow-up studies, we tested four possible signals that users might use to decide how much to trust an app---data collection, quality of reputation, presence of ads, and occurrence of payment---and found that all four signals affected trust. %We also identified several demographic features that are correlated with trust. 
A summary of the statistical evidence validating these effects is given in Figure~\ref{fig:signals->trust}.


\subsubsection{Data Collection Affects Trust}
% Annabel's experiment
In our second full user study, participants were told what types of data were collected by the app and asked how trustworthy they would consider the app. Participants were randomly assigned to one of four conditions that corresponded to different levels of data collection: MinimumNecessary, WithoutAds, WithAds, and AllData. The full methodology is described in Section~\ref{subsec:collection->trust}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/collection-to-trust.png}
    \caption{Reported Trust Level for Different Amounts of Data Collection}
    \label{fig:collection->trust}
\end{figure}

\begin{figure}[t]
\begin{center}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
 Collection & MinNec & WithoutAds & WithAds & AllData \\
 \hline
 MinNec & NA & 8.42e-09 & 1.46e-10 & 3.15e-10\\ 
 WithoutAds & & NA & 0.30 & .72 \\ 
 WithAds &  &  & NA & 0.07 \\ 
 AllData &  &  &  & NA \\ 
 \hline
\end{tabular}
\caption{\label{table:collection->trust-pvals} $p$-values from Pairwise Chi2 Contingency Tests for Statistically Significant Differences in Reported Trust Level for Different Amounts of Data Collection}
\end{center}
\end{figure}

We found that most participants assigned to the MinimumNecessary condition rated the app very trustworthy (38\%) or somewhat trustworthy (40\%), whereas in other conditions only a small minority (10-18\%) of participants rated the app to be either very trustworthy or somewhat trustworthy. Conversely, 70\% of the participants assigned to the AllData condition rated the app very untrustworthy, whereas 46-56\% of participants selected this response in the WithAds and WithoutAds conditions, and just 7\% selected this response in the MinimumNecessary condition. Assigning each trust level a numeric score (1 for very untrustworthy up to 5 for very trustworthy), we found that the average trust level monotonically decreased as the amount of data collected increased: MinimumNecessary (1 data type collected) had an average trust level of 3.96, WithoutAds (5 data types collected) had an average trust level of 1.92, WithAds (10 data types collected) had an average trust level of 1.83, and AllData (19 data types collected) had an average trust level of 1.63. The complete data about reported trust levels is shown in Figure~\ref{fig:collection->trust}. 

When participants were made aware of data collection by an app, it had a significant effect on how trustworthy they felt the app to be. We ran a linear regression (input: assessment, output: trust) which yielded $R^2 = 0.4061$, suggesting that data collection condition explains around 40\% of the variation in trust. Finally, we performed pairwise chi-squared contingency tests to determine whether there were statistically significant differences between the distribution of reported trust levels for each condition. We found that the MinimumNecessary condition was significantly different from the other conditions ($p<.001$), which we confirmed with a Bonferroni correction ($\alpha = .008$). However, the other pairwise tests did not find statistically significant differences. The complete results are shown in Table~\ref{table:collection->trust-pvals}.




\subsubsection{App Reputation Affects Trust}

Our third user study, described in Section~\ref{subsect:reputation->trust}, investigated whether app reputation---a composite attribute that includes quality of reviews, publisher reputation, app store verification, number of downloads, and other similar factors---influences how trustworthy a user deems an app to be. 

Our five conditions corresponded to linear manipulations of the individual features, so we expected to see a linear correlation between the quality of reputation and users' level of trust; our results, depicted in Figure~\ref{fig:reputation->trust}, validated this hypothesis. Pairwise chi-squared contingency tests found statistically significant differences between each of the distributions of trust level. We also performed a linear regression using the reputation level, and we found that reputation affected approximately 22\% of the variation in how trustworthy the user considered the app to be (Figure~\ref{fig:signals->trust}). 

% EB Note: I'm not sure whether we want to include info about data collection
%Using the above qualitative results describing features people use to assess their level of trust in an app, we ran an experiment in which we manipulated those features in order to indirectly manipulate people's trust in a hypothetical app. We hypothesized that doing so would reveal a linear trend relating level of trust to privacy assessment, but were surprised to find a different result. As shown in Figure~\ref{fig:uShapeCurve}, participants assigned to the highest and lowest trust conditions thought the application collected more data than in all the other conditions.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/reputation-to-trust.png}
    \caption{Frequency of Different Reported Trust Levels for Different Reputation Levels}
    \label{fig:reputation->trust}
\end{figure}

\begin{figure}[t]
\begin{center}
{\small 
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
 Reputation & 1 & 2 & 3 & 4 & 5 \\
 \hline
 1 & NA & 2.00e-10 & 2.08e-19& 1.99e-32 & 2.93e-31 \\ 
 2 & & NA   & 0.000518 & 6.50e-11 & 3.49e-14\\ 
  3 &  &  & NA & 0.00695 & 3.64e-08\\ 
 4 &  &  &   & NA & 0.00161\\ 
 4 &  &  &   & & NA \\ 
 \hline
\end{tabular}
}
\caption{\label{table:ads-payment->trust-pvals} $p$-values from Pairwise Chi2 Contingency Tests for Statistically Significant Differences in Reported Trust Level for Different Reputation Levels}
\end{center}
\end{figure}

\subsubsection{Advertising affects Trust}
\label{subsec:results:ads->trust}


In our final user study, we tested for the effect of advertising on user trust, both in the presence and in the absence of payment. Participants were randomly assigned to one of four conditions: FreeWithAds, FreeWithoutAds, PaidWithAds, or BuyOutAds; the full methodology is described in Section~\ref{subsec:ads-payment->trust}.

In the conditions where no payment occurred, we found that fewer participants considered a free app with ads to be very trustworthy or somewhat trustworthy (50\%) compared to a free app without ads (66\%), and more participants considered a free app with ads to be very untrustworthy or somewhat untrustworthy (20\%) compared to a free app without ads (9\%). We observed the same effect in the conditions in which payment occurred. The complete results are shown in Figure~\ref{fig:ads-payment->trust}. We also performed pairwise chi-squared tests and found that the distribution of reported trust levels was significantly different in the conditions with ads versus the conditions without ads, both when no payment occurred and when payment occurred ($p < .0001$). Finally, we performed a linear regression (combining the two conditions with ads and the two conditions without ads) and found that the presence of advertising decreases the reported user trust level, and that advertising explains about 4\% of that trust level (Figure~\ref{fig:signals->trust}). 


%As secondary analyses, we also analyzed the distribution of trust by partitioning trust into ``low'' and ``high'' trust buckets (e.g., 1 vs 2-5, 1-2 vs 3-5, 1-3 vs 4-5, 1-4 vs 5) and comparing distributions of high and low trust responses using chi-squared tests, and by treating trust as a continuous variable and comparing its mean in different conditions using T-tests. All of these tests also had convincing p-values and effects pointing in the same direction.


%Combining the date from the two conditions with advertising (WithAds and PaidWithAds) and the two conditions without advertising (WithoutAds and BuyoutAds), we performed a linear regression and found that the presence of adverting decreases the level of user trust and that advertising explains about 4\% of a user's trust level. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/ads-payment-to-trust.png}
    \caption{Frequency of Different Reported Trust Levels in the Presence and Absence of Advertising and Payment}
    \label{fig:ads-payment->trust}
\end{figure}

\begin{figure}[t]
\begin{center}
{\small 
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
\multirow{2}{*}{Condition} & \multicolumn{2}{|c|}{Free} & \multicolumn{2}{|c|}{Paid} \\
\cline{2-5}
  &WithAds & NoAds  & WithAds & BuyOutAds\\
 \hline
 FreeWithAds & NA & 3.21e-09  & 0.000124& 0.159\\ 
 FreeNoAds & & NA  & 3.08-19 & 0.000243\\ 
  PaidWithAds &  &  & NA & 3.36e-08 \\ 
 BuyOutAds &  &  &   & NA \\ 

 \hline
\end{tabular}
}
\caption{\label{table:ads-payment->trust-pvals} $p$-values from Pairwise Chi2 Contingency Tests for Statistically Significant Differences in Reported Trust Level for Game Apps With and Without Advertising and/or Payment}
\end{center}
\end{figure}


\subsubsection{Payment Affects Trust}

We also analysed the effect of payment on user trust. Our initial observations found that more participants consider the app very untrustworthy or somewhat untrustworthy when payment occurred, both when the app contained ads (33\% vs 20\%) and when the app did not contain ads (17\% vs. 9\%). Similarly, fewer participants found the app very trustworthy or somewhat trustworthy when payment occurred, both when the app contained ads (40\% vs. 50\%) and when the app did not contain ads (56\% vs. 62\%). The complete results are shown in Figure~\ref{fig:ads-payment->trust}.

The negative effect of payment on trust level is consistent with the qualitative results reported in our third pilot study but the opposite of our original hypothesis; we had expected the occurrence of payment to be positively correlated with trust due to an expectation of buying privacy. The statistical significance of this inverse correlation was upheld by our statistical analysis. We performed pairwise chi-squared contingency tests and found that the distribution of reported trust levels was significantly different between the conditions in which payment occurred compared to the conditions in which no payment occurred, both when the app contained ads ($p=.000124$) and when the app did not contain ads ($p=.000243$). Finally, we performed a linear regression (combining the two conditions with payment and the two conditions without payment) and found that the occurrence of payment explains about 1.6\% of a user's trust level. 


We also looked at the interaction between payment and advertising. Upon visual examination, we noted that the fraction of responses that deemed the app untrustworthy in the PaidWithAds condition appears to be substantially higher (33\%) than in the other three conditions (less than 20\%); the fraction of trustworthy responses in this condition also appears to be substantially lower (38\%) than in the other three conditions (greater than 50\%); these differences in distribution are all statistically significant (Figure~\ref{table:ads-payment->trust-pvals}). We hypothesize that this is due to the fact that paid game apps with advertising are unusual in the real-world and thus this combination seemed suspicious to our participants. Conversely, the distribution of responses for the BuyOutAds condition is statistically indistinguishable from the FreeWithAds condition (likely due to the opposing effects of advertising and payment), negating our initial hypothesis that paying to remove ads would be seen by users as paying for additional trustworthiness (and less data collection). 
    


\begin{figure}[t]
    \centering
    \begin{tabular}{ |c|c|c|c| } 
    \hline
    \textbf{Predictor} & \textbf{p-value} &	\textbf{$R^2$}	& \textbf{Adjusted $R^2$} \\
    \hline
    collection & 2.00E-16 &	0.4061 & 0.3971\\
    reputation &	2.00E-16 &	0.2201 &	0.2193\\
    ads	& 6.18E-16 &	0.04057	& 0.03996\\
    pay & 2.57E-07 &	0.01668	& 0.01605\\
    ads+pay	& 2.20E-16 &	0.05928 &	0.05809\\
     \hline
    \end{tabular}
    \caption{A summary of results from linear regressions testing how strongly different signals predict trust.}
    \label{fig:signals->trust}
\end{figure}


\subsection{Demographic Effects on Trust}

\begin{figure*}
\begin{center}
\begin{tabular}{ |c|c|c|c|c| } 
\hline
\textbf{Predictor} & \textbf{Study} & \textbf{p-value} &	\textbf{	$R^2$}	& \textbf{Adjusted $R^2$} \\
\hline\hline
\multirow{3}{*}{Age} & User Study 2 (Data Collection) &	0.108	& 0.4289	& 0.4082\\
& User Study 3 (Reputation) &	\textit{0.00509}$^{*}$	& 0.2324	& 0.228\\
& User Study 4 (Ads+Payment)	 & 0.333 & 0.06202 & 0.05844\\
\hline
\multirow{3}{*}{Gender}  & User Study 2 (Data Collection)  & 0.208 & 0.4109 & 0.3989\\
& User Study 3 (Reputation) & 0.306 & 0.2218 & 0.2196\\
& User Study 4 (Ads+Payment)	 &	\textit{0.00532}$^{*}$	& 0.06684	& 0.06388\\
\hline
\multirow{3}{*}{Sexual Orientation} & User Study 2 (Data Collection)  	& 0.414	& 0.4181	& 0.3969\\
& User Study 3 (Reputation) 	& \textit{0.0139}$^{*}$	& 0.2293	& 0.2256\\
& User Study 4 (Ads+Payment)	 & 0.229 & 0.06264 & 0.05906\\
\hline
\multirow{3}{*}{Social Views} & User Study 2 (Data Collection)  	& \textit{0.027}$^{*}$	& 0.4387	& 0.4184\\
& User Study 3 (Reputation) 	& \textit{0.00614}$^{*}$	& 0.06784	& 0.06429\\
& User Study 4 (Ads+Payment)		& \textit{0.00334}$^{**}$	& 0.2317	& 0.228\\
\hline
\multirow{3}{*}{Religious Views} & User Study 2 (Data Collection)  	& 0.402	& 0.4183	& 0.3972\\
& User Study 3 (Reputation) 	& \textit{0.00478}$^{**}$	& 0.2311	& 0.2274\\
& User Study 4 (Ads+Payment)		& \textit{0.000105}$^{**}$	& 0.07316	& 0.06963\\
\hline
\multirow{3}{*}{Economic Views} & User Study 2 (Data Collection)   & \textit{0.0285}$^{*}$ & 0.4384 & 0.418\\
& User Study 3 (Reputation) & 0.874 & 0.221 & 0.2173\\
& User Study 4 (Ads+Payment)		& \textit{0.0481}$^{*}$	& 0.06499	& 0.06143\\
\hline
\multirow{3}{*}{Technical Background} & User Study 2 (Data Collection)  	& \textit{0.0237}$^{*}$	& 0.4214	& 0.4096\\
& User Study 3 (Reputation)  	& \textit{0.0000334}$^{**}$	& 0.2327	& 0.2313\\
& User Study 4 (Ads+Payment)		& 0.212	& 0.06021	& 0.05843\\
\hline
%\multirow{3}{*}{Application Use} & Collection 	& NA	& NA	& NA\\
% & Reputation 	& NA	& NA	& NA\\
%& Ads+Payment	& \textit{0.0026}$^{**}$	& 0.06636	& 0.06399\\
% \hline
\end{tabular}
\caption{Results of Statistical Tests for Correlations between Demographic Factors and Trust. $p$-values marked $^*$  are statistically significant ($p<.05$). $p$-values marked $^{**}$ are statistically significant after a Bonferroni correction ($\alpha = .005$). }
\label{fig:demographic-pvals}
\end{center}
\end{figure*}
For the three user studies that evaluated the effect of possible signals---data collection, reputation, and advertising/payment---we also tested for correlations between demographic factors and level of trust\footnote{Our first user study randomly assigned participants to different trust levels, and is therefore not included in this analysis.}. Demographic factors that were statistically significant in at least one of these studies are shown in Figure~\ref{fig:demographic-pvals}.

\paragraph{Basic Demographics} All basic demographics---including race, ethnicity, age, gender, and sexual orientation---tested negative for statistically significant effects in either all or or all but one of our surveys. Due to the large number of hypotheses tested, we suspect that the three factors that had statistically significant effects in one of the studies (age, gender, and sexual orientation) represent false positives (all three values are above the Bonferroni correction, $\alpha = .005$). We therefore conclude that there is no statistically significant effect of basic demographics on user trust.


\paragraph{Social Views} In all three user studies, we detected a statistically significant effect of social views on user trust.  Across all three studies, participants who identified as more socially conservative reported higher levels of trust. Due to the strong statistical effects of social views across all three surveys, we suspect that this effect is genuine and that users who identify as more socially conservative place more trust in mobile apps. 


\paragraph{Religious Views} In both large-scale user studies, we detected a statistically significant effect of religious views on user trust: users who self-identified as more religious were more likely to consider an app to be trustworthy. In the study that looked at the effect of data collection on trust, however, no statistically significant effect was detected ($p=.402$). Due to the smaller sample size in the survey about data collection and the strong statistical effects of the larger studies, we suspect that this effect is genuine: users who identify as more religious likely place more trust in mobile apps. We observe that this effect is consistent with known correlations between religious views and social views and with the effect of social views on trust (discussed above). 
    
\paragraph{Economic Views} In two of our user studies (data collection and ads+payment), we detected statistically significant effects of economic views on trust ($p<.05$): users who identified as more economically conservative placed more trust in the app. However, no statistically significant effect between economic views and trust was detected the study that investigated the effect of app reputation, and the tests with lower $p$-values were still above the Bonferroni correction value ($\alpha = .005$). Nonetheless, we observe that the two studies in which effects were detected either explicitly or implicitly relate to economic views---both ads, payment, and data collection are all potential revenue sources for mobile apps---so it is possible that these studies prompted users to incorporate their economic views more carefully into their trust assessment. We therefore consider these results to be inconclusive: further research will be required to determine whether economic views affect trust. 
     
\paragraph{Technical Background} We expected users with more technical background to report lower levels of trust. However, we found the opposite effect in both studies where technical background was significant; users with more technical background reported higher levels of trust in mobile apps. Instead of our original hypothesis, perhaps respondents with technical backgrounds have trust levels founded based on more accurate information about privacy than respondents without technical backgrounds. However, we consider these results to be inconclusive: further research will be required to determine whether economic views affect trust.
    
Overall, our results suggest that most demographics have no effect or only a small effect on user trust. Social views and religious views appear to be correlated with trust assessments, but basic demographics seem to have no effect on trust. From the data we collected, it is unclear whether economic views or technical background affect trust, but we suspect that any such effect, if it exists, is likely small. 






==> sections/50-trust-data.tex <==

\section{Follow-up Study: Trustworthiness and Data Collection}
\label{sec:discussion:trustCausesData}
    
This work explores the relationship between user perception of signals (advertising and payment) and user beliefs about data collection and trust. However, it is also natural to explore whether a causal relationship exists between users' trust in apps and their assessments of data collection by those apps. %Our random assignment of conditions in our full study allowed us to ascribe causal relationships between our signals (ads and payment) and assessment of data collection and trustworthiness, but those  experiments  cannot determine whether a causal relationship exists between users' trust in apps and their assessments of data collection. 
     
We hypothesize that trust seems likely to be an important factor in how users assess the privacy properties of apps. Perhaps trust intermediates the effects of various other proxies. For example, perhaps the presence of ads causes users to trust an app less, which in turn causes them to believe that the app collects more data. Such a model could explain how a variety of other factors, beyond ads and payment, influence assessment of data collection mediated through trust. We believe that further exploration of the role of trust is an important next step.

Beginning on that path, we conducted a follow-up study in which we attempted to directly manipulate trust as a randomized condition variable

    
\begin{comment} 
\begin{figure}
\begin{center}
{\small
\begin{tabular}{ |c||c|c|c|c|c| } 
 \hline
 \parbox{1cm}{\centering Trust } & \parbox{1cm}{\centering Very \\ Untrust.} & \parbox{1cm}{\centering Some.\\ Untrust.} & \parbox{1cm}{\centering Neither} & \parbox{1cm}{\centering Some. \\Trust.} & \parbox{1cm}{\centering Very \\Trust.} \\ 
 \hline
 \hline
 \parbox{1cm}{\centering Very \\ Untrust.} & NA & 0.002 & <.001 & <.001 & <.001\\ 
 \hline
 \parbox{1cm}{\centering Some.\\ Untrust.} & & NA & <.001 & <.001 & <.001\\
 \hline
 \parbox{1cm}{\centering Neither} &  &  & NA & 0.670 & 0.427\\
 \hline
 \parbox{1cm}{\centering Some. \\Trust.} &  &  &  & NA & 0.222\\
 \hline
 \parbox{1cm}{\centering Very \\Trust.} &  &  &  &  & NA\\ 
 \hline
\end{tabular}
}
\caption{Results of Two-sample t-test p-values for Different Assigned Trusts}
\label{table:pairwise-pvals}
\end{center}
\end{figure}
\end{comment}

\subsection{Methodology} 
To determine whether the level of trust a user places in a mobile app affects that user's beliefs about data collection practices by the app, we conducted a user study with 545 users in which we directly manipulated the trust level. Respondents recruited through Amazon Mechanical Turk; to participate in the study, users were required to be located in the US and to have previously completed at least 50 HITs with an approval rate of at least 95\%.

Each participant was assigned to one of five conditions corresponding to different trust levels: very untrustworthy, somewhat untrustworthy, neither trustworthy nor untrustworthy, somewhat trustworthy, very trustworthy. Each participant was told to imagine that they had discovered a new game app and had decided it was that trustworthy; on the same page they were asked, ``In this scenario, what words are used to describe how trustworthy you consider this app?'' (our attention-check question). Participants were then asked to indicate whether they thought that each of the 19 data types (identified in our first pilot) would be collected by that app. For each type of data, the participant could select yes, no, or only in certain cases (e.g., if I give permission or if I click a button). For each type of data that the participant indicated would be collected, the participant was then asked to select the purpose of the data collection. The survey concluded with questions about the participant's technical background and demographics. The full survey is included in Appendix~\ref{appendix:trust->collection}.

We read through each of the responses to the attention check question and rejected 42 responses that were deemed unrelated to or inconsistent with the specified level of trust; we then analysed the remaining 503 responses. The median completion time was 3.6 minutes; respondents who successfully completed the survey were paid $\$.70$. 

%Demographically,  9.34\% of our population were 18-24, 43.14\% were 25-34, 27.24\% were 35-44, 15.11\% were 45-59, 4.77\% were 60-74, and .40\%  were 75 or older. Racially, 80.72\% of our respondents were white, 14.71\% were black or African American, 1.19\% were American Indian or Alaska Native, 4.77\% were Asian, .60\% were Pacific Islander or Native Hawaiian, and .80\% were another race.\footnote{The numbers do not sum to 100\% because respondents were allowed to select more than one race.} 53.08\% of the respondents identified as men, 46.72\% as women, .20\% as non-binary, and 0\% selected ``Other.'' A graphical summary of these demographics---along with a comparison to the demographics of our other studies and to the demographics of the United States as published in the American Community Survey---is depicted in Figure~\ref{fig:demographics}. 

%We observe briefly that the demographics of these user studies are not an exact match to the overall demographics of the United States; notably, our sample population is notably younger that the overall population, a known property of the Amazon Mechanical Turk worker pool~\cite{ipeirotis2010demographics}. However, prior work has found that Mechanical Turk results for surveys on security and privacy topics generalize well despite the demographic discrepancy, particularly for populations under 50 with at least some college education~\cite{redmiles2019well}. \linebreak




    \begin{figure}[t!]
       \includegraphics[width = \columnwidth]{figures/assessmentByTrust.pdf}
       \caption{Effect of direct trust manipulation on assessment of data collection (out of 19 possible types of data). In low trust conditions, we observed higher amounts of assessed data collection, but in the other conditions differences in trust appeared to have no effect on assessment of data collection. Green triangles show the mean, yellow lines show the median, boxes show interquartile range, and whiskers show from 5\% to 95\%.}
       \label{fig:AssessmentByTrust}
    \end{figure}

\subsection{Results}


We found that participants assigned to low-trust conditions (somewhat untrustworthy and very untrustworthy) assumed that significantly more unnecessary data collection would occur compared to participants assigned to high-trust conditions (somewhat trustworthy and very trustworthy). Participants in low-trust conditions predicted an average of 7.94/19 types of data would be unnecessarily collected, whereas participants in high-trust conditions predicted an average of 4.01/19 types of data would be unnecessarily collected. We used a two-sample t-test to confirm that these means are significantly different ($p<.001$). \footnote{We chose to use t-tests as they are robust to the normality assumption, particularly with large sample sizes, which were present in this study. As possible data points are limited in range (maximum 19 pieces of data to be collected) there were also few outliers that could significantly affect t-tests, further making them a good choice.} 
% TODO: add numbers to this paragraph
% Question: did we run a regression on this?
% Consider adding a just somewhat un vs both trustworthy




Notably, participants assigned to the very untrustworthy condition assessed particularly high levels of data collection compared to the other conditions. The mean number of data types assessed by participants in this condition was $35\%$ higher than in the next-highest (somewhat untrustworthy) condition, and is confirmed to be significantly different using two-sample t-test ($p<.001$). Moreover, 75\% of participants in the very untrustworthy condition inferred that at least 6 different types of data were collected, whereas for all other conditions, the 75th percentile was no more than two types of data. We hypothesize that this might imply certain underlying beliefs, such as the belief that only ``sketchy'' or actively malicious apps are likely to collect large amounts of data. 


However, there were not statistically significant differences between the two high-trust conditions ($p=0.222$) or between the combined high-trust conditions (very trustworthy somewhat trustworthy) and the neutral condition ($p=0.811$). We hypothesize that the diminished effect of trust on assessment at higher trust levels might be due to the fact that our studies looked specifically at game apps: users might place an a priori upper bound on the level of trustworthiness they ascribe to game apps. Thus our participants, who were told that the app in question was a game, may be likely to be reasoning from a compressed scale of internal feelings about trustworthiness. This hypothesis is consistent with the results from the study looking at the effect of ads and payment, which found that just $8.33\%$ of participants who were shown screenshots from a real-world mobile game app (a free app containing ads) rated that app as very trustworthy. % (a complete description of the results of that study is available in Section~\ref{subsec:results:ads->trust}).


We also found that the neutral trust condition did not fit the trend defined by the four non-neutral conditions. % This is not a technically meaningful sentence. TODO: discuss whether there are statistics to support this story. 
We hypothesize that participants in this condition might be interpreting the phrase ``neither trustworthy nor trustworthy'' ambiguously, imposing assumptions about the general trustworthiness of apps more strongly than in other conditions.

\subsection{Discussion}

 These results suggest that for less trustworthy apps, differences in trust cause significantly different assessment. For ``very untrustworthy'' apps, the median assessment was 9 unique types of data collected, for ``somewhat untrustworthy apps'' it was 7 unique types of data collected, for all other conditions (``neither trustworthy nor untrustworthy'', ``somewhat trustworthy'', and ``very trustworthy''), the median was 3-4 data types. These preliminary results are depicted in Figure~\ref{fig:AssessmentByTrust}. We intend to continue and expand this work in scope and in rigor to better determine both the influence on trust of a variety of factors such as app popularity, ratings, publisher, nationality, and more, as well as to better constrain the effects of trust---and of factors outside of trust---on users' perceptions of data collection.
    
 

==> sections/57-discussion.tex <==
%\section{Trust and Data Collection}

%This work explores the relationship between user perception of signals (advertising and payment), data collection, and trust. Our results provide insight into the connections between these factors and also highlight issues relating to data collection and privacy.
    
\begin{comment} 
    
    % 1. Known real-world connection between advertising and data collection. People are (appropriately) using advertising as a signal about data collection. Maybe heartening? People are picking up on a real trend. Useful inferences are happening.
    \subsection{Proxy Signals and Informed Consent} We observe that past work~\cite{stevens2012,book2013longitudinal} indicates that the presence of advertising \emph{does} in fact correlate with greater data collection. This means that users' reliance on ads as a proxy for data collection is, in some sense, reasonable and warranted. Users may thus be making more informed decisions by using signals to assess data collection which actually correlate with data collection.
    
    However, individual accuracy at assessing which data types were collected by our two apps (Woody Puzzle and Infinite Word search) was still very low.
    
    We did expert readings of the privacy policies of both apps to establish a ground-truth of the data collected by each app. Additionally, we read the privacy policies of ad libraries embedded by the apps. We broke down the data collected by an app into two categories: data collected directly by the app, and data collected by ad libraries embedded in the app. The data collected directly by the app was considered to be the ground truth of how much data would be collected for conditions without ads. We took the union of an app's individual collection with its ad libraries' collection to determine the ground truth of how much data would be collected in conditions with ads. We found that Woody Puzzle collected 8 (resp., 7) types of data with (resp., without) ads, and that Infinite Word Search collected 7 (resp., 3) types of data with (resp., without). 
    
    Overall, our respondents had an accuracy of $.674$ in predicting which data types were collected by the app they were shown. However, this number is influenced by the number of data types that were (correctly predicted) not collected by these apps. If we only consider data types collected by the app, users correctly identified that those data types were collected only 55.1\% of the time, a rate that is not much higher than guessing at random. Moreover, there was no significant difference in users' assessment of data collection between the two apps ($p=0.166$), which highlights the fact that correlations inherently fail to capture the particular data collection practices of individual apps, particularly those that deviate from the norm.  
    
    Based on these results, we believe that the use of proxy signals---even ones that strongly correlate with actual data collection---should not be considered a sufficient basis for informed consent, or as evidence that the app ecosystem is behaving appropriately with respect to privacy. While these heuristics lean the right way, they rarely match the specifics of data collection practices. These specifics are often extremely important to users, especially for users for whom privacy is a matter of safety. For example, specific types of data, such as location data or contact information, may be highly sensitive for specific groups, such as survivors of intimate partner violence~\cite{freed2018stalker}. Thus for many people, a general impression of the quantity of data collected by an app may be less important than the specific types of data collected. 
    
    Additionally, participants were unable to accurately predict differences in data collection practices between the two game apps in our study. Our results are compatible, therefore, with the idea that users are ``stereotyping'' apps using clues such as the presence of ads and, perhaps, the genre of the app. Apps which choose to collect less data are unlikely to be rewarded with a competitive advantage if users employing proxies are unable to detect or guess at which apps are more or less privacy preserving, and apps which choose to collect more data will do so without users' awareness or informed consent.
 \end{comment}
 
    % 2. Role of trust - what else is influencing trust? Is there a causal relationship between trust and assessment? Can present preliminary results from follow-up studies
    \section{Trust and Data Collection}
    \label{sec:discussion:trustCausesData}
    
    This work explores the relationship between user perception of signals (advertising and payment) and user beliefs about data collection and trust. However, it is also natural to explore whether a causal relationship exists between users' trust in apps and their assessments of data collection by those apps. Our random assignment of conditions in our full study allowed us to ascribe causal relationships between our signals (ads and payment) and assessment of data collection and trustworthiness, but those 
     the experiments  cannot determine whether a causal relationship exists between users' trust in apps and their assessments of data collection. 
     
     We hypothesize that trust seems likely to be an important factor in how users assess the privacy properties of apps. Perhaps trust intermediates the effects of various other proxies. For example, perhaps the presence of ads causes users to trust an app less, which in turn causes them to believe that the app collects more data. Such a model could explain how a variety of other factors, beyond ads and payment, influence assessment of data collection mediated through trust.

    \begin{figure}[t!]
       \includegraphics[width = \columnwidth]{figures/assessmentByTrust.pdf}
       \caption{Effect of direct trust manipulation on assessment of data collection (out of 19 possible types of data). In low trust conditions, we observed higher amounts of assessed data collection, but in the other conditions differences in trust appeared to have no effect on assessment of data collection. Green triangles show the mean, yellow lines show the median, boxes show interquartile range, and whiskers show from 5\% to 95\%.}
       \label{fig:AssessmentByTrust}
    \end{figure}

    We believe that further exploration of the role of trust is an important next step. Beginning on that path, we conducted a preliminary study in which we attempted to directly manipulate trust as a randomized condition variable, by using specific wording to describe apps as more or less trustworthy. These results suggest that for less trustworthy apps, differences in trust cause significantly different assessment. For ``very untrustworthy'' apps, the median assessment was 9 unique types of data collected, for ``somewhat untrustworthy apps'' it was 7 unique types of data collected, for all other conditions (``neither trustworthy nor untrustworthy'', ``somewhat trustworthy'', and ``very trustworthy''), the median was 3-4 data types. These preliminary results are depicted in Figure~\ref{fig:AssessmentByTrust}. We intend to continue and expand this work in scope and in rigor to better determine both the influence on trust of a variety of factors such as app popularity, ratings, publisher, nationality, and more, as well as to better constrain the effects of trust---and of factors outside of trust---on users' perceptions of data collection.
    
    
    % 3. Mental models of privacy, payments, and app profit models
    \subsection{Payment and Data Collection} 
    Our findings of a non-linear amplification effect of payment surprised us by refuting our simpler hypothesis that occurrence of payment, like absence of advertisement, would be associated directly with the perception of reduced data collection. While our results cannot fully explain the causes of this effect, we present here one model we believe to be compatible with the findings of both our main study (Section~\ref{sec:results}) and of our preliminary study described in the prior paragraph on trust and data collection (Section~\ref{sec:discussion:trustCausesData}).
    
    We hypothesize that users believe apps profit in one of two ways: either apps monetize user data, or they charge users directly. Under this ``buying privacy'' model, users would believe that payment indicates lower levels of data collection, since direct payment negates the needs to make money by monetizing user data. We hypothesize that this signal may in fact be present in the data, showing itself in the fact that for apps with no ads, the presence of payment was associated with a belief that less data was collected. 
    
    Further, we hypothesize that this signal may be covered up when ads are present in the app, because the combination of ads and payment drive trust low enough that the effects of trust dominate over the effects of the ``buying privacy'' model alone. In our preliminary study of the effects of trust on assessment (Section~\ref{sec:discussion:trustCausesData}), low trust caused users to believe that 2-3x data was collected when compared to neutral and high levels of trust. In our main results, we found that apps with both ads and payment were considered significantly less trustworthy.
    In particular, significantly more users rated the conditions with ads to be very or somewhat untrustworthy (Figure~\ref{fig:trustByCondition}), levels where trust causes very large increases in assessment of data collected. The buying privacy effect may be present here, but it is dominated by the effects of trust. Meanwhile, on the high end, variations in trust have no effect on data collection assessment, since we found no difference in assessment when apps were considered neutrally trustworthy or better. Thus in this situation, the ``buying privacy'' theory shines through and explains why users believed that even less data was collected in scenarios with both payment and ads.
    
        
    
    % Thus in the combination of these models, the amplification effect on one end is caused by a ``buying privacy'' model, while the amplification effect on the other end is caused by a reduction in trust due to the use of payment
    % Considering our actual results, we suggest that perhaps users possess a more complex mental model---or a set of multiple mental models between which they switch for different apps---of the profit models of apps. 
    % For example, users might associate payment with a decrease in data collection by trustworthy apps and also believe that very untrustworthy or ``sketchy'' apps collect more data; since the paid game apps with ads were seen as less trustworthy, the combination of these two mental models could explain the amplifying effect of payment we observed. 
    
    This model is one possible explanation. While compatible with our results, it is best viewed as a hypothesis to be further explored by future work. We believe that exploring people's beliefs and mental models about the profit models of apps, and the inferences they make about data collection based on those mental models, could be a valuable future direction toward understanding the full suite of features that people use to assess the privacy properties of the apps they use. Such modeling could be invaluable to evaluating the ways in which informed consent may be failing to uphold a  well-functioning privacy ecosystem.
    

 \begin{comment}   
    \input{sections/55-limitations}
    
\end{comment}
% We talked about adding a results section looking at purpose to determine mental model questions -- probably too much for the time we have.






% \begin{comment}
% % EB Note: I'm not sure that we still want to include this stuff...
% Given that advertising affects user beliefs about data collection, we then evaluated how well users infer actual data collection practices given this signal. We generated a ground truth for data collection through an expert close reading of the relevant privacy policies. We defined the ground truth for the conditions without ads based on the data collection practices disclosed in the application privacy policies, and we defined the ground trust for the conditions with ads by combining the data collection practices in the application privacy policies with those of the ad libraries disclosed by the application developer. Overall, our respondents had an accuracy of $.701$. 



% We view these results as an indication that mobile app users are surprisingly well-informed about data collection practices by mobile apps despite the fact that these users do not read and understand posted privacy policies. Nonetheless, further work will be required to explore other possible signals such as genre or design quality and to extend these results beyond the domain of mobile game applications.



% However, these results do not necessarily imply that informed consent is sufficient for privacy. We observe that users had significantly better accuracy predicting data collection practices for the Infinite Word Search/FreeNoAds condition ($.727$) than for the the Woody Puzzle/FreeNoAds condition ($.686$). In fact, data collection predictions were indistinguishable between the two conditions ($p=??$) despite the fact that their data collection practices are different (Woody Puzzle collects 7 different types of data while Infinite Word Search collects only 3). That is, user perceptions appear to reflect norms about app behavior (conditioned on certain signals) and do not capture distinctions between individual apps. As a result, privacy expectations might be better met by a regime that enforces limitations based on social norms, such as contextual integrity~\cite{Nissenbaum09} or use-based privacy~\cite{Cate06}, than by the current practice of notice and consent. 
% \end{comment}


==> sections/XX-introduction-CI.tex <==
\section{Introduction}

Prior work has conclusively demonstrated that notice and consent is not an effective mechanism for guaranteeing privacy~\cite{refs}. Contextual Integrity~\cite{nissenbaum2004privacy,Niss09,Niss11} provides an alternative approach for how to provide meaningful user privacy: privacy is defined by cultural norms around data collection, and privacy is violated when data use practices are inconsistent with those norms. However, effectly ensuring privacy by leveraging contextual integrity depends on accurately understanding data collection norms in a particular context.

In this work, we investigate U.S. cultural norms around data collection by mobile game apps. 
%Although there is much work identifying users' mental models of threats and individuals' security and privacy perceptions and behaviors (e.g.,~\cite{malhotra_internet_2004,nissenbaum2004privacy,egelman2015scaling,Wash2010FolkMO,kang2015,Lin2012ExpectationAP}), there has been little examination of what factors influence which principals come to be perceived as security or privacy threats. 
We consider two possible signals that have been found to be correlated with actual data use practices: advertising~\cite{stevens2012,book2013longitudinal} and price (free vs. paid)~\cite{saborido2017comprehension,han2020,bamberger2020}. Prior work has found that these signals in combination affect user perceptions of apps in various ways (e.g., users expect that a paid, ad-free version of the app will have better security and privacy behaviors than a free, ad-supported app~\cite{han2020,bamberger2020}); this work takes the next step by exploring how each of these signals individually impact user expectations about data collection by mobile apps. We also consider a third signal---timing of payment---that is not known to correlate with actual data use practices, but for which typical app behavior has changed over time (away from paying for an ad-free version of an app and towards making an in-app purchase to remove ads from an ad-supported free app).
%
We conducted and online user survey ($n=2109$) to explore how user-visible signals impact social norms about data collection. % whether these signals persuade users that a mobile app should be perceived as a \emph{privacy threat}, which we characterize as an principal that is perceived as both (1) untrustworthy and (2) having access to personal information. Thus our studies measured changes in perceived trustworthiness and perceived data collection by apps in order to operationalize perceptions of apps as privacy threats.

%To evaluate how each of these factors individually affect user beliefs, we ran a 2109-person study on Amazon Mechanical Turk. Participants were randomly assigned to one of five conditions; four of these conditions correspond to the presence or absence of our two independent signals: whether or not there are ads in the app and whether that app was free or paid. The final condition corresponds to the case where a user initially installs a free version of the app and then pays to remove ads. In each condition, the participant was shown a story comprising a series of screenshots of a mobile app with brief descriptions describing their interactions with that app. The respondent was then shown a list of nineteen different data types (determined by a pilot study) and asked to rate how likely it was that the app would collect that type of data. The respondent was also asked to rate the trustworthiness of the app. 

Our first research question is: how do each of our signals (presence of ads, occurrence of payment, timing of payment) individually affect social norms about data collection? We found that respondents who were assigned to the conditions with ads expected apps to collect more personal data, but that  presence or absence of payment alone did not have a significant impact on users' expectations. We also found that users were not able to accurately assess which data types were collected by a particular app. While conducting this analysis, we also observed that  many users hold misconceptions about what data is collected (and by whom) for the purpose of payment processing. %Overall, 24.7\% of users incorrectly believed that one or more data types was collected by the app for the purpose of processing payments. Naturally, this misconception was most common in conditions that included payment  and for data types commonly entered during online payments (e.g., credit card information, mailing address, phone number). When we re-analyzed our data after correcting for this misconception, we observed the same results: ads significantly impacted users' assessment of data collection but payment alone did not. However, we did observe a significant interaction between advertising and payment. 

%Next, we analyzed our user responses to determine whether these signals affect user beliefs about how trustworthy an application is. Again we found that users considered apps with ads to be significantly less trustworthy than apps without ads. We also found that there was a significant interaction between ads and payment. Users were less likely to consider an app trustworthy when shown the condition with a paid app with ads (PaidWithAds), compared to users who were shown a free app with ads (FreeWithAds). The majority of users who were shown a free app without ads (FreeNoAds) considered it trustworthy, and an even larger portion of users who were shown a paid app without ads (PaidNoAds) did so; all differences were statistically significant. 




Second, we found evidence to disprove our timing hypothesis. We found that users expected apps that initially contained ads to collect significantly more data after paying to remove ads from a previously installed app compared to an (ad-free) app they had initially paid for. %This belief held even after correcting for the misconceptions about payment processing. %Users were also significantly less likely to consider an app trustworthy after they had paid to remove ads compared to an app that they had initially purchased without ads. 

%Finally we conducted a follow-up study ($n=545$) to further explore the relationship between our two dimensions of privacy threat: amount of data collected and trustworthiness. Our results suggest that for less trustworthy apps, perceptions of trustworthiness are used as a proxy to make inferences about the amount of data collected by an app. 


We view the key contributions of this work as:
\begin{enumerate}
    \item Identifying and experimentally validating three factors---advertising, payment, and timing of payment---that might impact the contextual integrity of mobile apps.
    \item Establishing U.S. social norms about data collection by mobile game apps. 
    \item Identifying and quantifying misconceptions about how data is collected in order to process payments.
    \item Making recommendations for how to leverage social norms to enhance privacy for the mobile game ecosystem. 
\end{enumerate}

Further work will be required to determine whether there exist other factors that influence user assessment and to extend the scope beyond game apps. Nonetheless, we view this work as an important step in providing a more nuanced understanding of social norms and contextual integrity for mobile apps. 









